Data-driven shape inference in three-dimensional steady state supersonic flows using ODIL and JAX-Fluids

We present a novel data- and first-principles-driven method for inferring the shape of a solid obstacle and its flow field in three-dimensional steady-state supersonic flows. The method combines the Optimizing a Discrete Loss (ODIL) technique with the automatically differentiable JAX-Fluids CFD solver to jointly reconstruct flow fields and obstacle shapes. ODIL minimizes the discrete residual of the governing PDE via gradient descent-based algorithms and inherits the consistency and stability of the chosen numerical discretization. Discrete residuals and their gradients are computed using JAX-Fluids, which features nonlinear shock-capturing schemes and level-set-based immersed solid boundaries. We validate our method on synthetic data for challenging inverse problems, including shape inference of solid obstacles in 3D steady-state supersonic flows. In particular, we study flow around a cylinder, sphere, and ellipse. Two shape representations are investigated: (1) parametric, where the shape is described by a small set of parameters (e.g., radius of the cylinder or sphere) optimized jointly with the flow field, and (2) free-form, where the level-set function is optimized pointwise over the mesh without predefined shapes. For the parametric case, we provide a detailed comparison with Physics-Informed Neural Networks. We demonstrate that the combination of nonlinear shock-capturing discretization and level-set-based interface representation enables accurate inference of obstacle shapes and flow fields via the ODIL method. This approach opens new avenues for solving complex inverse problems in supersonic aerodynamics.

==> figures/flow_field_reconstruction/error_table.tex <==
\begingroup
\pgfkeys{/pgf/number format/.cd, sci, precision=2, zerofill}

% compressionramp
\pgfplotstableread{./figures/flow_field_reconstruction/compressionramp/error_history_30000.txt}\datatable
\pgfplotstablegetrowsof{\datatable}
\pgfmathtruncatemacro{\lastrow}{\pgfplotsretval-1}
\pgfplotstablegetelem{\lastrow}{[index]0}\of\datatable
\pgfmathsetmacro{\rhoc}{\pgfplotsretval}
\pgfplotstablegetelem{\lastrow}{[index]1}\of\datatable
\pgfmathsetmacro{\pc}{\pgfplotsretval}
\pgfplotstablegetelem{\lastrow}{[index]3}\of\datatable
\pgfmathsetmacro{\uc}{\pgfplotsretval}
\pgfplotstablegetelem{\lastrow}{[index]4}\of\datatable
\pgfmathsetmacro{\vc}{\pgfplotsretval}

% expansionramp
\pgfplotstableread{./figures/flow_field_reconstruction/expansionramp/error_history_30000.txt}\datatable
\pgfplotstablegetrowsof{\datatable}
\pgfmathtruncatemacro{\lastrow}{\pgfplotsretval-1}
\pgfplotstablegetelem{\lastrow}{[index]0}\of\datatable
\pgfmathsetmacro{\rhoe}{\pgfplotsretval}
\pgfplotstablegetelem{\lastrow}{[index]1}\of\datatable
\pgfmathsetmacro{\pe}{\pgfplotsretval}
\pgfplotstablegetelem{\lastrow}{[index]3}\of\datatable
\pgfmathsetmacro{\ue}{\pgfplotsretval}
\pgfplotstablegetelem{\lastrow}{[index]4}\of\datatable
\pgfmathsetmacro{\ve}{\pgfplotsretval}

\begin{table}[!t]
  \centering
  \begin{tabular}{r c c c c}
    \hline
    Shape&$\rho$ & $u$ & $v$ & $p$ \\
    \hline
    Expansion ramp&\print{\rhoe}&\print{\ue}&\print{\ve}&\print{\pe} \\
    Compression ramp&\print{\rhoc}&\print{\uc}&\print{\vc}&\print{\pc} \\
    \hline
  \end{tabular}
  \caption{
    Mean cell-wise absolute relative error between the ODIL
    and reference solution for the flow field inference from known obstacle shapes.
    }
  \label{tab:error_known_shapes}
\end{table}

\endgroup

==> figures/flow_field_reconstruction/flowfield_p_M.tex <==
\begin{tikzpicture}
    % \pgfmathdeclarefunction{lg10}{1}{%
    %     \pgfmathparse{ln(#1)/ln(10)}%
    % }
    
    % Spectral_r colormap from matplotlib
    \pgfplotsset{
        colormap={spectralr}{rgb255=(94,79,162) rgb255=(68,112,177) rgb255=(59,146,184) rgb255=(89,180,170)
            rgb255=(126,203,164) rgb255=(166,219,164) rgb255=(202,233,157) rgb255=(232,246,156) 
            rgb255=(247,252,179) rgb255=(254,245,175) rgb255=(254,227,145) rgb255=(253,200,119) 
            rgb255=(252,170,95) rgb255=(247,131,77) rgb255=(236,97,69) rgb255=(218,70,76)
            rgb255=(190,36,73) rgb255=(158,1,66)}}
    
    \begin{groupplot}[
        group style={
            group size=4 by 3,
            horizontal sep=0.8cm,
            vertical sep=0.5cm
        }, 
        width=4.2cm, 
        height=4.2cm
        ]
        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            title=$p$,
            ylabel=ODIL,
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/flow_field_reconstruction/compressionramp/pressure_30000_xy_odil.pdf};


        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            title=$Ma$,
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/flow_field_reconstruction/compressionramp/machnumber_30000_xy_odil.pdf};

        
        \nextgroupplot[
            xshift=0.5cm,
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            title=$p$,
            enlargelimits=false,
            colormap name=spectralr,
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/flow_field_reconstruction/expansionramp/pressure_30000_xy_odil.pdf};

        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            title=$Ma$,
            enlargelimits=false,
            colormap name=spectralr,
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/flow_field_reconstruction/expansionramp/machnumber_30000_xy_odil.pdf};


        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            ylabel=reference,
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image,
            colorbar,
            colorbar horizontal,
            colorbar style={
                at={(0.0,-0.05)},
                % yshift=0.3cm,
                anchor=north west,
                xtick style={
                    draw=none,
                },
                xtick={1.00,1.39,1.78},
                xticklabels = {1.00,1.39,1.78},
                height=0.3cm
            },
            point meta min=1.0,
            point meta max=1.78
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/flow_field_reconstruction/compressionramp/pressure_30000_xy_ref.pdf};


        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image,
            colorbar,
            colorbar horizontal,
            colorbar style={
                at={(0.0,-0.05)},
                % yshift=0.3cm,
                anchor=north west,
                xtick style={
                    draw=none,
                },
                xtick={1.63,1.815,2.00},
                xticklabels = {1.63,1.815,2.00},
                height=0.3cm
            },
            point meta min=1.63,
            point meta max=2.00
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/flow_field_reconstruction/compressionramp/machnumber_30000_xy_ref.pdf};

        
        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            enlargelimits=false,
            colormap name=spectralr,
            colorbar,
            colorbar horizontal,
            colorbar style={
                at={(0.0,-0.05)},
                % yshift=0.3cm,
                anchor=north west,
                xtick style={
                    draw=none,
                },
                xtick={0.46,0.73,1.00},
                xticklabels = {0.46,0.73,1.00},
                height=0.3cm
            },
            point meta min=0.46,
            %point meta max=0.5188506842
            point meta max=1.00
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/flow_field_reconstruction/expansionramp/pressure_30000_xy_ref.pdf};

        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            enlargelimits=false,
            colormap name=spectralr,
            colorbar,
            colorbar horizontal,
            colorbar style={
                at={(0.0,-0.05)},
                % yshift=0.3cm,
                anchor=north west,
                xtick style={
                    draw=none,
                },
                xtick={2.00,2.23,2.46},
                xticklabels = {2.00,2.23,2.46},
                height=0.3cm
            },
            point meta min=2.00,
            point meta max=2.46
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/flow_field_reconstruction/expansionramp/machnumber_30000_xy_ref.pdf};


        \nextgroupplot[
            yshift=-0.5cm,
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            ylabel=$\log_{10}(\vert\text{rel. error}\vert)$,
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image,
            colorbar,
            colorbar horizontal,
            colorbar style={
                at={(0.0,-0.05)},
                % yshift=0.3cm,
                anchor=north west,
                xtick style={
                    draw=none,
                },
                xtick={-5,-3,-1},
                % xticklabels = {-4,-3,-2},
                height=0.3cm
            },
            point meta min=-5,
            point meta max=-1
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/flow_field_reconstruction/compressionramp/pressure_30000_xy_error.pdf};


        \nextgroupplot[
            yshift=-0.5cm,
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image,
            colorbar,
            colorbar horizontal,
            colorbar style={
                at={(0.0,-0.05)},
                % yshift=0.3cm,
                anchor=north west,
                xtick style={
                    draw=none,
                },
                xtick={-5,-3,-1},
                % xticklabels = {-4,-3,-2},
                height=0.3cm
            },
            point meta min=-5,
            point meta max=-1
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/flow_field_reconstruction/compressionramp/machnumber_30000_xy_error.pdf};

        
        \nextgroupplot[
            yshift=-0.5cm,
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            enlargelimits=false,
            colormap name=spectralr,
            colorbar,
            colorbar horizontal,
            colorbar style={
                at={(0.0,-0.05)},
                % yshift=0.3cm,
                anchor=north west,
                xtick style={
                    draw=none,
                },
                xtick={-5,-3,-1},
                % xticklabels = {-4,-3,-2},
                height=0.3cm
            },
            point meta min=-5,
            point meta max=-1
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/flow_field_reconstruction/expansionramp/pressure_30000_xy_error.pdf};

        \nextgroupplot[
            yshift=-0.5cm,
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            enlargelimits=false,
            colormap name=spectralr,
            colorbar,
            colorbar horizontal,
            colorbar style={
                at={(0.0,-0.05)},
                % yshift=0.3cm,
                anchor=north west,
                xtick style={
                    draw=none,
                },
                xtick={-5,-3,-1},
                % xticklabels = {-4,-3,-2},
                height=0.3cm
            },
            point meta min=-5,
            point meta max=-1
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/flow_field_reconstruction/expansionramp/machnumber_30000_xy_error.pdf};
    \end{groupplot}
    \node[above, yshift=1cm] at ($(group c1r1.north east)!0.5!(group c2r1.north west)$) {Compression ramp};
    \node[above, yshift=1cm] at ($(group c3r1.north east)!0.5!(group c4r1.north west)$) {Expansion ramp};
\end{tikzpicture}


==> figures/flow_field_reconstruction/flowfield_rho_u.tex <==
\begin{tikzpicture}
    % \pgfmathdeclarefunction{lg10}{1}{%
    %     \pgfmathparse{ln(#1)/ln(10)}%
    % }
    
    % Spectral_r colormap from matplotlib
    \pgfplotsset{
        colormap={spectralr}{rgb255=(94,79,162) rgb255=(68,112,177) rgb255=(59,146,184) rgb255=(89,180,170)
            rgb255=(126,203,164) rgb255=(166,219,164) rgb255=(202,233,157) rgb255=(232,246,156) 
            rgb255=(247,252,179) rgb255=(254,245,175) rgb255=(254,227,145) rgb255=(253,200,119) 
            rgb255=(252,170,95) rgb255=(247,131,77) rgb255=(236,97,69) rgb255=(218,70,76)
            rgb255=(190,36,73) rgb255=(158,1,66)}}
    
    \begin{groupplot}[
        group style={
            group size=4 by 3,
            horizontal sep=0.8cm,
            vertical sep=0.5cm
        }, 
        width=4.2cm, 
        height=4.2cm
        ]
        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            title=$\rho$,
            ylabel=ODIL,
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/flow_field_reconstruction/compressionramp/density_30000_xy_odil.pdf};


        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            title=$u$,
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/flow_field_reconstruction/compressionramp/velocityX_30000_xy_odil.pdf};

        
        \nextgroupplot[
            xshift=0.5cm,
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            title=$\rho$,
            enlargelimits=false,
            colormap name=spectralr,
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/flow_field_reconstruction/expansionramp/density_30000_xy_odil.pdf};

        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            title=$u$,
            enlargelimits=false,
            colormap name=spectralr,
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/flow_field_reconstruction/expansionramp/velocityX_30000_xy_odil.pdf};


        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            ylabel=reference,
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image,
            colorbar,
            colorbar horizontal,
            colorbar style={
                at={(0.0,-0.05)},
                % yshift=0.3cm,
                anchor=north west,
                xtick style={
                    draw=none,
                },
                xtick={1.00,1.24,1.48},
                xticklabels = {1.00,1.24,1.48},
                height=0.2cm
            },
            point meta min=1.0,
            point meta max=1.48
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/flow_field_reconstruction/compressionramp/density_30000_xy_ref.pdf};


        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image,
            colorbar,
            colorbar horizontal,
            colorbar style={
                at={(0.0,-0.05)},
                % yshift=0.3cm,
                anchor=north west,
                xtick style={
                    draw=none,
                },
                xtick={2.06,2.21,2.36},
                xticklabels = {2.06,2.21,2.36},
                height=0.2cm
            },
            point meta min=2.06,
            point meta max=2.36
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/flow_field_reconstruction/compressionramp/velocityX_30000_xy_ref.pdf};

        
        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            enlargelimits=false,
            colormap name=spectralr,
            colorbar,
            colorbar horizontal,
            colorbar style={
                at={(0.0,-0.05)},
                % yshift=0.3cm,
                anchor=north west,
                xtick style={
                    draw=none,
                },
                xtick={0.54,0.77,1.00},
                xticklabels = {0.54,0.77,1.00},
                height=0.2cm
            },
            point meta min=0.54,
            %point meta max=0.5188506842
            point meta max=1.00
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/flow_field_reconstruction/expansionramp/density_30000_xy_ref.pdf};

        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            enlargelimits=false,
            colormap name=spectralr,
            colorbar,
            colorbar horizontal,
            colorbar style={
                at={(0.0,-0.05)},
                % yshift=0.3cm,
                anchor=north west,
                xtick style={
                    draw=none,
                },
                xtick={2.37,2.47,2.57},
                xticklabels = {2.37,2.47,2.57},
                height=0.2cm
            },
            point meta min=2.37,
            %point meta max=2.3842830658
            point meta max=2.57
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/flow_field_reconstruction/expansionramp/velocityX_30000_xy_ref.pdf};


        \nextgroupplot[
            yshift=-0.5cm,
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            ylabel=$\log_{10}(\vert\text{rel. error}\vert)$,
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image,
            colorbar,
            colorbar horizontal,
            colorbar style={
                at={(0.0,-0.05)},
                % yshift=0.3cm,
                anchor=north west,
                xtick style={
                    draw=none,
                },
                xtick={-5,-3,-1},
                % xticklabels = {-4,-3,-2},
                height=0.2cm
            },
            point meta min=-5,
            point meta max=-1
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/flow_field_reconstruction/compressionramp/density_30000_xy_error.pdf};


        \nextgroupplot[
            yshift=-0.5cm,
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image,
            colorbar,
            colorbar horizontal,
            colorbar style={
                at={(0.0,-0.05)},
                % yshift=0.3cm,
                anchor=north west,
                xtick style={
                    draw=none,
                },
                xtick={-5,-3,-1},
                % xticklabels = {-4,-3,-2},
                height=0.2cm
            },
            point meta min=-5,
            point meta max=-1
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/flow_field_reconstruction/compressionramp/velocityX_30000_xy_error.pdf};

        
        \nextgroupplot[
            yshift=-0.5cm,
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            enlargelimits=false,
            colormap name=spectralr,
            colorbar,
            colorbar horizontal,
            colorbar style={
                at={(0.0,-0.05)},
                % yshift=0.3cm,
                anchor=north west,
                xtick style={
                    draw=none,
                },
                xtick={-5,-3,-1},
                % xticklabels = {-4,-3,-2},
                height=0.2cm
            },
            point meta min=-5,
            point meta max=-1
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/flow_field_reconstruction/expansionramp/density_30000_xy_error.pdf};

        \nextgroupplot[
            yshift=-0.5cm,
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            enlargelimits=false,
            colormap name=spectralr,
            colorbar,
            colorbar horizontal,
            colorbar style={
                at={(0.0,-0.05)},
                % yshift=0.3cm,
                anchor=north west,
                xtick style={
                    draw=none,
                },
                xtick={-5,-3,-1},
                % xticklabels = {-4,-3,-2},
                height=0.2cm
            },
            point meta min=-5,
            point meta max=-1
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/flow_field_reconstruction/expansionramp/velocityX_30000_xy_error.pdf};
    \end{groupplot}
    \node[above, yshift=1cm] at ($(group c1r1.north east)!0.5!(group c2r1.north west)$) {Compression ramp};
    \node[above, yshift=1cm] at ($(group c3r1.north east)!0.5!(group c4r1.north west)$) {Expansion ramp};
\end{tikzpicture}


==> figures/flow_field_reconstruction/loss_history.tex <==
\begin{tikzpicture}

    \begin{groupplot}[
        group style={group size=2 by 1, horizontal sep=2.5cm},
        width=4.2cm, height=4.2cm]
      

    \nextgroupplot[
        tick align=outside,
        tick pos=left,
        legend style={at={(1.2,1.1)},draw=black,anchor=north east,font=\footnotesize,legend columns=2},
        xtick style={color=black},
        ymin=1e-10, ymax=1e4,
        % xmin=0.0, xmax=1e5,
        log basis x={10},
        log basis y={10},
        % xmode=log,
        ymode=log,
        xlabel=step,
        ylabel=$\omega \mathcal{L}$,
        title=Compression ramp
        % ylabel=$\mathcal{L}$
        ]
    
    \addplot [line width=1.0pt, TUMblue] table[skip first n=1,
    x index = {0}, y index = {2}
    ] {figures/flow_field_reconstruction/compressionramp/loss_history_30000.txt};
    \addlegendentry{$E$};
    \addplot [line width=1.0pt, TUMorange] table[skip first n=1,
        x index = {0}, y index = {3}
        ] {figures/flow_field_reconstruction/compressionramp/loss_history_30000.txt};
    \addlegendentry{$W$};
    \addplot [line width=1.0pt, TUMgreen] table[skip first n=1,
        x index = {0}, y index = {4}
        ] {figures/flow_field_reconstruction/compressionramp/loss_history_30000.txt};
    \addlegendentry{$S$};
    \addplot [line width=1.0pt, TUMgray] table[skip first n=1,
        x index = {0}, y index = {6}
        ] {figures/flow_field_reconstruction/compressionramp/loss_history_30000.txt};
    \addplot [line width=1.0pt, black, dashed] coordinates {(10000,1e-12) (10000,1e4)};
    \addlegendentry{$T_0$};
    % \addplot [line width=1.0pt, black, dotted] coordinates {(20000,1e-12) (20000,1e4)};

    \nextgroupplot[
    tick align=outside,
    tick pos=left,
    xtick style={color=black},
    ymin=1e-12, ymax=1e4,
    % xmin=0.0, xmax=1e5,
    log basis x={10},
    log basis y={10},
    % xmode=log,
    ymode=log,
    xlabel=step,
    title=Expansion ramp
    ]

    \addplot [line width=1.0pt, TUMblue] table[skip first n=1,
        x index = {0}, y index = {2}
        ] {figures/flow_field_reconstruction/expansionramp/loss_history_30000.txt};
    \addplot [line width=1.0pt, TUMorange] table[skip first n=1,
        x index = {0}, y index = {3}
        ] {figures/flow_field_reconstruction/expansionramp/loss_history_30000.txt};
    \addplot [line width=1.0pt, TUMgreen] table[skip first n=1,
        x index = {0}, y index = {4}
        ] {figures/flow_field_reconstruction/expansionramp/loss_history_30000.txt};
    \addplot [line width=1.0pt, TUMgray] table[skip first n=1,
        x index = {0}, y index = {6}
        ] {figures/flow_field_reconstruction/expansionramp/loss_history_30000.txt};
    \addplot [line width=1.0pt, black, dashed] coordinates {(10000,1e-12) (10000,1e4)};
    % \addplot [line width=1.0pt, black, dotted] coordinates {(20000,1e-12) (20000,1e4)};


    \end{groupplot}
\end{tikzpicture}

==> figures/free_shape_inference/comparison.tex <==
\begin{tikzpicture}
    % \pgfmathdeclarefunction{lg10}{1}{%
    %     \pgfmathparse{ln(#1)/ln(10)}%
    % }
    
    % Spectral_r colormap from matplotlib
    \pgfplotsset{
        colormap={spectralr}{rgb255=(94,79,162) rgb255=(68,112,177) rgb255=(59,146,184) rgb255=(89,180,170)
            rgb255=(126,203,164) rgb255=(166,219,164) rgb255=(202,233,157) rgb255=(232,246,156) 
            rgb255=(247,252,179) rgb255=(254,245,175) rgb255=(254,227,145) rgb255=(253,200,119) 
            rgb255=(252,170,95) rgb255=(247,131,77) rgb255=(236,97,69) rgb255=(218,70,76)
            rgb255=(190,36,73) rgb255=(158,1,66)}}
    
    \begin{groupplot}[
        group style={
            group size=4 by 3,
            horizontal sep=0.2cm,
            vertical sep=0.5cm
        }, 
        width=4.6cm, 
        height=4.6cm
        ]
        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            title style={align=center},
            title={Integrated \\ inferred shape},
            ylabel=Cylinder,
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image,
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/free_shape_inference/comparison_time_stepping/cylinder_density_forward.pdf};


        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            title=reference,
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image,
            colorbar,
            colorbar,
            colorbar style={
                at={(1.05,0.0)},
                % yshift=0.3cm,
                anchor=south west,
                ytick style={
                    draw=none,
                },
                ytick={0.07,1.56,3.05},
                yticklabels = {0.07,1.56,3.05},
                width=0.2cm
            },
            point meta min=0.07,
            point meta max=3.05
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/free_shape_inference/comparison_time_stepping/cylinder_density_ref.pdf};

        
        \nextgroupplot[
            xshift=1.5cm,
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            title style={align=center},
            title={Integrated \\ inferred shape},
            enlargelimits=false,
            colormap name=spectralr,
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/free_shape_inference/comparison_time_stepping/cylinder_velocityX_forward.pdf};

        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            title=reference,
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image,
            colorbar,
            colorbar style={
                at={(1.05,0.0)},
                % yshift=0.3cm,
                anchor=south west,
                ytick style={
                    draw=none,
                },
                ytick={-0.32,1.1,2.52},
                yticklabels = {-0.32,1.1,2.52},
                width=0.2cm
            },
            point meta min=-0.32,
            point meta max=2.52
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/free_shape_inference/cylinder/odil/velocityX_50000_xy_ref.pdf};





        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            ylabel=Ellipse,
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image,
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/free_shape_inference/comparison_time_stepping/ellipse_density_forward.pdf};


        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image,
            colorbar,
            colorbar style={
                at={(1.05,0.0)},
                % yshift=0.3cm,
                anchor=south west,
                ytick style={
                    draw=none,
                },
                ytick={0.07,1.55,3.03},
                yticklabels = {0.07,1.55,3.03},
                width=0.2cm
            },
            point meta min=0.07,
            point meta max=3.03
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/free_shape_inference/comparison_time_stepping/ellipse_density_ref.pdf};

        
        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            enlargelimits=false,
            colormap name=spectralr,
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/free_shape_inference/comparison_time_stepping/ellipse_velocityX_forward.pdf};

        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image,
            colorbar,
            colorbar style={
                at={(1.05,0.0)},
                % yshift=0.3cm,
                anchor=south west,
                ytick style={
                    draw=none,
                },
                ytick={0.01,1.27,2.53},
                yticklabels = {0.01,1.27,2.53},
                width=0.2cm
            },
            point meta min=0.01,
            point meta max=2.53
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/free_shape_inference/ellipse/odil/velocityX_50000_xy_ref.pdf};






        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            ylabel=Sphere,
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image,
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/free_shape_inference/comparison_time_stepping/sphere_density_forward.pdf};


        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image,
            colorbar,
            colorbar style={
                at={(1.05,0.0)},
                % yshift=0.3cm,
                anchor=south west,
                ytick style={
                    draw=none,
                },
                ytick={0.12,1.47,2.82},
                yticklabels = {0.12,1.47,2.82},
                width=0.2cm
            },
            point meta min=0.12,
            point meta max=2.82
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/free_shape_inference/comparison_time_stepping/sphere_density_ref.pdf};

        
        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            enlargelimits=false,
            colormap name=spectralr,
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/free_shape_inference/comparison_time_stepping/sphere_velocityX_forward.pdf};

        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image,
            colorbar,
            colorbar style={
                at={(1.05,0.0)},
                % yshift=0.3cm,
                anchor=south west,
                ytick style={
                    draw=none,
                },
                ytick={-0.52,1.01,2.54},
                yticklabels = {-0.52,1.01,2.54},
                width=0.2cm
            },
            point meta min=-0.52,
            point meta max=2.54
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/free_shape_inference/sphere/odil/velocityX_30000_xy_ref.pdf};


    \end{groupplot}

    % \node[above] at ($(group c1r1.north)$) {ODIL shape + time stepping};
    % \node[above] at ($(group c3r1.north)$) {ODIL shape + time stepping};
    % \node[above, yshift=1cm] at ($(group c3r1.north east)!0.5!(group c4r1.north west)$) {$u$};
\end{tikzpicture}


==> figures/free_shape_inference/flowfield_rho_u1.tex <==
\begin{tikzpicture}
    % \pgfmathdeclarefunction{lg10}{1}{%
    %     \pgfmathparse{ln(#1)/ln(10)}%
    % }
    
    % Spectral_r colormap from matplotlib
    \pgfplotsset{
        colormap={spectralr}{rgb255=(94,79,162) rgb255=(68,112,177) rgb255=(59,146,184) rgb255=(89,180,170)
            rgb255=(126,203,164) rgb255=(166,219,164) rgb255=(202,233,157) rgb255=(232,246,156) 
            rgb255=(247,252,179) rgb255=(254,245,175) rgb255=(254,227,145) rgb255=(253,200,119) 
            rgb255=(252,170,95) rgb255=(247,131,77) rgb255=(236,97,69) rgb255=(218,70,76)
            rgb255=(190,36,73) rgb255=(158,1,66)}}
    
    \begin{groupplot}[
        group style={
            group size=6 by 3,
            horizontal sep=0.1cm,
            vertical sep=0.5cm
        }, 
        width=3.9cm, 
        height=3.9cm
        ]
        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            title=ODIL,
            % ylabel=Cylinder,
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image,
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/free_shape_inference/cylinder/odil/density_50000_xy_odil.pdf};


        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            title=reference,
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/free_shape_inference/cylinder/odil/density_50000_xy_ref.pdf};


        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            title style={align=center},
            title={ODIL shape \\ time stepping solution},
            % ylabel=Cylinder,
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image,
            colorbar,
            colorbar style={
                at={(1.05,0.0)},
                % yshift=0.3cm,
                anchor=south west,
                ytick style={
                    draw=none,
                },
                ytick={0.07,1.56,3.05},
                yticklabels = {0.07,1.56,3.05},
                width=0.2cm
            },
            point meta min=0.07,
            point meta max=3.05
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/free_shape_inference/comparison_time_stepping1/cylinder_density_forward.pdf};


        \nextgroupplot[
            % xshift=1.5cm,
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            % title=ODIL,
            enlargelimits=false,
            colormap name=spectralr,
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/free_shape_inference/cylinder/odil/velocityX_50000_xy_odil.pdf};


        \nextgroupplot[
            % xshift=1.5cm,
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            % title=ODIL,
            enlargelimits=false,
            colormap name=spectralr,
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/free_shape_inference/cylinder/odil/velocityX_50000_xy_ref.pdf};


        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            % title=reference,
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image,
            colorbar,
            colorbar style={
                at={(1.05,0.0)},
                % yshift=0.3cm,
                anchor=south west,
                ytick style={
                    draw=none,
                },
                ytick={-0.32,1.1,2.52},
                yticklabels = {-0.32,1.1,2.52},
                width=0.2cm
            },
            point meta min=-0.32,
            point meta max=2.52
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/free_shape_inference/comparison_time_stepping1/cylinder_velocityX_forward.pdf};





        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            % ylabel=Ellipse,
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image,
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/free_shape_inference/ellipse/odil/density_50000_xy_odil.pdf};

        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            % ylabel=Ellipse,
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image,
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/free_shape_inference/ellipse/odil/density_50000_xy_ref.pdf};

        
        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image,
            colorbar,
            colorbar style={
                at={(1.05,0.0)},
                % yshift=0.3cm,
                anchor=south west,
                ytick style={
                    draw=none,
                },
                ytick={0.07,1.55,3.03},
                yticklabels = {0.07,1.55,3.03},
                width=0.2cm
            },
            point meta min=0.07,
            point meta max=3.03
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/free_shape_inference/comparison_time_stepping1/ellipse_density_forward.pdf};

        
        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            enlargelimits=false,
            colormap name=spectralr,
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/free_shape_inference/ellipse/odil/velocityX_50000_xy_odil.pdf};

        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            enlargelimits=false,
            colormap name=spectralr,
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/free_shape_inference/ellipse/odil/velocityX_50000_xy_ref.pdf};

        
        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image,
            colorbar,
            colorbar style={
                at={(1.05,0.0)},
                % yshift=0.3cm,
                anchor=south west,
                ytick style={
                    draw=none,
                },
                ytick={0.01,1.27,2.53},
                yticklabels = {0.01,1.27,2.53},
                width=0.2cm
            },
            point meta min=0.01,
            point meta max=2.53
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/free_shape_inference/comparison_time_stepping1/ellipse_velocityX_forward.pdf};


        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            % ylabel=Sphere,
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image,
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/free_shape_inference/sphere/odil/density_30000_xy_odil.pdf};

        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            % ylabel=Sphere,
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image,
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/free_shape_inference/sphere/odil/density_30000_xy_ref.pdf};


        \nextgroupplot[
            tick align=outside,
            tick pos=left,
            xtick style={draw=none},
            ytick style={draw=none},
            xticklabels = {},
            xtick = {},
            yticklabels = {},
            ytick = {},
            enlargelimits=false,
            colormap name=spectralr,
            axis equal image,
            colorbar,
            colorbar style={
                at={(1.05,0.0)},
                % yshift=0.3cm,
                anchor=south west,
                ytick style={
                    draw=none,
                },
                ytick={0.12,1.47,2.82},
                yticklabels = {0.12,1.47,2.82},
                width=0.2cm
            },
            point meta min=0.12,
            point meta max=2.82
        ]
        \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/free_shape_inference/comparison_time_stepping1/sphere_density_forward.pdf};

        
        % \nextgroupplot[
        %     tick align=outside,
        %     tick pos=left,
        %     xtick style={draw=none},
        %     ytick style={draw=none},
        %     xticklabels = {},
        %     xtick = {},
        %     yticklabels = {},
        %     ytick = {},
        %     enlargelimits=false,
        %     colormap name=spectralr,
        % ]
        % \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/free_shape_inference/sphere/odil/velocityX_30000_xy_odil.pdf};

        % \nextgroupplot[
        %     tick align=outside,
        %     tick pos=left,
        %     xtick style={draw=none},
        %     ytick style={draw=none},
        %     xticklabels = {},
        %     xtick = {},
        %     yticklabels = {},
        %     ytick = {},
        %     enlargelimits=false,
        %     colormap name=spectralr,
        %     axis equal image,
        %     colorbar,
        %     colorbar style={
        %         at={(1.05,0.0)},
        %         % yshift=0.3cm,
        %         anchor=south west,
        %         ytick style={
        %             draw=none,
        %         },
        %         ytick={-0.52,1.01,2.54},
        %         yticklabels = {-0.52,1.01,2.54},
        %         width=0.2cm
        %     },
        %     point meta min=-0.52,
        %     point meta max=2.54
        % ]
        % \addplot graphics [xmin=-0.3,xmax=0.3,ymin=-0.3,ymax=0.3] {figures/free_shape_inference/sphere/odil/velocityX_30000_xy_ref.pdf};


    \end{groupplot}

    % \node[above, yshift=1cm] at ($(group c1r1.north east)!0.5!(group c2r1.north west)$) {$\rho$};
    % \node[above, yshift=1cm] at ($(group c3r1.north east)!0.5!(group c4r1.north west)$) {$u$};
\end{tikzpicture}


==> figures/free_shape_inference/measurement_noise/error_table.tex <==
\begingroup
\pgfkeys{/pgf/number format/.cd, sci, precision=2, zerofill}

\pgfplotstableread{./figures/free_shape_inference/cylinder/odil/error_history_50000.txt}\datatable
\pgfplotstablegetrowsof{\datatable}
\pgfmathtruncatemacro{\lastrow}{\pgfplotsretval-1}
\pgfplotstablegetelem{\lastrow}{[index]0}\of\datatable
\pgfmathsetmacro{\rhoa}{\pgfplotsretval}
\pgfplotstablegetelem{\lastrow}{[index]1}\of\datatable
\pgfmathsetmacro{\pa}{\pgfplotsretval}
\pgfplotstablegetelem{\lastrow}{[index]3}\of\datatable
\pgfmathsetmacro{\ua}{\pgfplotsretval}
\pgfplotstablegetelem{\lastrow}{[index]4}\of\datatable
\pgfmathsetmacro{\va}{\pgfplotsretval}

\pgfplotstableread{./figures/free_shape_inference/measurement_noise/10/error_history_50000.txt}\datatable
\pgfplotstablegetrowsof{\datatable}
\pgfmathtruncatemacro{\lastrow}{\pgfplotsretval-1}
\pgfplotstablegetelem{\lastrow}{[index]0}\of\datatable
\pgfmathsetmacro{\rhob}{\pgfplotsretval}
\pgfplotstablegetelem{\lastrow}{[index]1}\of\datatable
\pgfmathsetmacro{\pb}{\pgfplotsretval}
\pgfplotstablegetelem{\lastrow}{[index]3}\of\datatable
\pgfmathsetmacro{\ub}{\pgfplotsretval}
\pgfplotstablegetelem{\lastrow}{[index]4}\of\datatable
\pgfmathsetmacro{\vb}{\pgfplotsretval}

\pgfplotstableread{./figures/free_shape_inference/measurement_noise/20/error_history_50000.txt}\datatable
\pgfplotstablegetrowsof{\datatable}
\pgfmathtruncatemacro{\lastrow}{\pgfplotsretval-1}
\pgfplotstablegetelem{\lastrow}{[index]0}\of\datatable
\pgfmathsetmacro{\rhoc}{\pgfplotsretval}
\pgfplotstablegetelem{\lastrow}{[index]1}\of\datatable
\pgfmathsetmacro{\pc}{\pgfplotsretval}
\pgfplotstablegetelem{\lastrow}{[index]3}\of\datatable
\pgfmathsetmacro{\uc}{\pgfplotsretval}
\pgfplotstablegetelem{\lastrow}{[index]4}\of\datatable
\pgfmathsetmacro{\vc}{\pgfplotsretval}

\pgfplotstableread{./figures/free_shape_inference/measurement_noise/30/error_history_50000.txt}\datatable
\pgfplotstablegetrowsof{\datatable}
\pgfmathtruncatemacro{\lastrow}{\pgfplotsretval-1}
\pgfplotstablegetelem{\lastrow}{[index]0}\of\datatable
\pgfmathsetmacro{\rhod}{\pgfplotsretval}
\pgfplotstablegetelem{\lastrow}{[index]1}\of\datatable
\pgfmathsetmacro{\pd}{\pgfplotsretval}
\pgfplotstablegetelem{\lastrow}{[index]3}\of\datatable
\pgfmathsetmacro{\ud}{\pgfplotsretval}
\pgfplotstablegetelem{\lastrow}{[index]4}\of\datatable
\pgfmathsetmacro{\vd}{\pgfplotsretval}

\begin{table}[!t]
  \centering
  \begin{tabular}{r c c c c c}
    \hline
    Noise in \%&$\rho$ & $u$ & $v$ &$p$ \\
    \hline
    0&\print{\rhoa}&\print{\ua}&\print{\va}&\print{\pa} \\
    10&\print{\rhob}&\print{\ub}&\print{\vb}&\print{\pb} \\
    20&\print{\rhoc}&\print{\uc}&\print{\vc}&\print{\pc} \\
    30&\print{\rhod}&\print{\ud}&\print{\vd}&\print{\pd} \\
    \hline
  \end{tabular}
  \caption{
    Mean cell-wise absolute relative error between ODIL
    and reference solution for
    free shape inference for
    different amount of noise
    on the primitive variable measurements.
    }
  \label{tab:errors_free_noise}
\end{table}

\endgroup

==> figures/schematic_flows.tex <==
\begin{tikzpicture}
    
    \coordinate (NULL) at (0,0);
    \def\L{4.5};
    \def\sepX{0.5}
    \coordinate (NULL_b) at ($(NULL) + (\L + \sepX,0)$);
    \coordinate (NULL_c) at ($(NULL) + (2*\L + 2*\sepX,0)$);
    
    \coordinate (CC) at ($(NULL) + (0.5*\L,0.5*\L)$);
    \draw[line width=1pt,->] (CC) -- ($(CC)+(0.5,0)$) node[at end, right] {$x$};
    \draw[line width=1pt,->] (CC) -- ($(CC)+(0,0.5)$) node[at end, above] {$y$};
    \draw[line width=1pt,->] (CC) -- ($(CC)+(0,0.5)$) node[at end, above] {$y$};

    % PLOT a)
    \def\sintheta{0.1736481777}; % corresponds to 10 deg
    \def\tantheta{0.1763269807}; % corresponds to 10 deg
    \def\cosbeta{0.7736854225}; % corresponds to 39 deg
    \def\sinbeta{0.6335699386}; % corresponds to 39 deg
    \coordinate (A) at (NULL);
    \coordinate (B) at ($(NULL) + (1*\L,0)$);
    \coordinate (C) at ($(NULL) + (1*\L,1*\L)$);
    \coordinate (D) at ($(NULL) + (0,1*\L)$);
  
    \node[below right, inner sep=5pt] at (D) {(a)};

    \coordinate (begin_ramp) at ($(0.16666*\L,0)$);
    \coordinate (end_ramp) at ($(1*\L,\sintheta*1.0*\L)$);
    \coordinate (end_shock) at ($(begin_ramp) + (0.8333*\L,\sinbeta/\cosbeta*0.8333*\L)$);
  
    \draw[line width=1pt] (A) rectangle (C);
    % \draw[line width=1pt] (begin_ramp) -- (end_ramp);
    \draw[line width=1pt] (begin_ramp.north east) -- (end_shock);
  
    % fill
    \filldraw[fill=black!10!white, line width=1pt] (begin_ramp.north) -- (B.north west) -- (end_ramp.west) -- (begin_ramp.north);
    \draw[<->, line width=0.5pt] ([xshift=-0.2cm]A) -- ([xshift=-0.2cm]D) node[midway, left] {0.6}; 
    \draw[<->, line width=0.5pt] ([yshift=0.2cm]D) -- ([yshift=0.2cm]C) node[midway, above] {0.6}; 
    \draw[<->, line width=0.5pt] ([yshift=0.2cm]A) -- ([yshift=0.2cm]begin_ramp) node[midway, above] {0.1}; 
    % \draw[line width=1pt] (A) rectangle (C);

    \draw pic[draw,red, "$\theta$", angle eccentricity=1.144,angle radius = 2.5cm] {angle = B--begin_ramp--end_ramp}; 
    \draw pic[draw,red, "$\lambda$", angle eccentricity=1.2,angle radius = 1.8cm] {angle = B--begin_ramp--end_shock}; 

    \coordinate (arrow_start) at ($0.3*(A) + 0.7*(D) + (0.1*\L,0)$);
    \draw[line width=1pt, ->] (arrow_start) -- node[above]{$M=2$} ($(arrow_start) + (0.15*\L,0)$);

    % PLOT b)

    \def\tanmu_1{0.5773502692}; % corresponds to 30 deg
    \def\tan_delta_mu_2{0.2640433588};

    \coordinate (A) at (NULL_b);
    \coordinate (B) at ($(NULL_b) + (1*\L,0)$);
    \coordinate (C) at ($(NULL_b) + (1*\L,1*\L)$);
    \coordinate (D) at ($(NULL_b) + (0,1*\L)$);
  
    \node[below right, inner sep=5pt] at (D) {(b)};

    \def\ramp_height{0.15 * \L};
    \def\length_vertical{0.15 * \L};
    \coordinate (E) at ($(A) + (0,\ramp_height)$);
    \coordinate (F) at ($(E) + (\L,0)$);
    \coordinate (begin_ramp) at ($(E) + (\length_vertical,0)$);
    \coordinate (end_ramp) at ($(begin_ramp) + (\ramp_height/\tantheta,-\ramp_height)$);
  
    \draw[line width=1pt] (A) rectangle (C);
    \draw[dashed, line width=1pt] (E) -- (F);

    % \draw[line width=1pt] (begin_ramp) -- ($(begin_ramp) + (0.85*\L/\tanmu_1,0.85*\L)$);
    \coordinate (end_rarefaction_1) at ($(begin_ramp) + (\L - \length_vertical, \L*\tanmu_1-\length_vertical*\tanmu_1)$);
    \draw[line width=1pt] (begin_ramp) -- (end_rarefaction_1);

    \coordinate (end_rarefaction_2) at ($(begin_ramp) + (\L - \length_vertical, \L*\tan_delta_mu_2-\length_vertical*\tan_delta_mu_2)$);
    \draw[line width=1pt] (begin_ramp) -- (end_rarefaction_2);

    % fill
    \filldraw[fill=black!10!white, line width=1pt] (E) -- (begin_ramp) -- (end_ramp) -- (A) -- (E);
    \draw[<->, line width=0.5pt] ([yshift=0.2cm]E) -- ([yshift=0.2cm]begin_ramp) node[midway, above] {0.1};
    % % \draw[line width=1pt] (A) rectangle (C);

    \draw pic[draw,red, "$\theta$", angle eccentricity=1.1,angle radius = 3.25cm] {angle = end_ramp--begin_ramp--F}; 
    \draw pic[draw,red, "$\mu_1$", angle eccentricity=1.2,angle radius = 1.75cm] {angle = F--begin_ramp--end_rarefaction_1}; 
    \draw pic[draw,red, "$\mu_2$", angle eccentricity=1.2,angle radius = 2.5cm] {angle = end_ramp--begin_ramp--end_rarefaction_2}; 
% 
    \coordinate (arrow_start) at ($0.3*(A) + 0.7*(D) + (0.1*\L,0)$);
    \draw[line width=1pt, ->] (arrow_start) -- node[above]{$M=2$} ($(arrow_start) + (0.15*\L,0)$);


    % PLOT c)
    \coordinate (A) at (NULL_c);
    \coordinate (B) at ($(NULL_c) + (1*\L,0)$);
    \coordinate (C) at ($(NULL_c) + (1*\L,1*\L)$);
    \coordinate (D) at ($(NULL_c) + (0,1*\L)$);

    \node[below right, inner sep=5pt] at (D) {(c)};

    \draw[line width=1pt] (A) rectangle (C);

    \draw[line width=1pt,fill=black!10!white] ($0.5*(A) + 0.5*(C)$) circle (0.1*\L);

    \coordinate (arrow_start) at ($0.3*(A) + 0.7*(D) + (0.1*\L,0)$);
    \draw[line width=1pt, ->] (arrow_start) -- node[above]{$M=2$} ($(arrow_start) + (0.15*\L,0)$);

    % \draw[thick] ($(A) + (0.8*\L,0)$) to[spline coordinates=S, spline through={($0.5*(A) + 0.5*(D)+ (0.2,0)$)($0.5*(A) + 0.5*(D)+ (0.2,0.1)$)}] ($(D) + (0.8*\L,0)$);
    \draw[line width=1pt] plot[smooth] coordinates {($(A) + (0.6*\L,0)$) ($0.5*(A) + 0.5*(D)+ (0.3*\L,0)$) ($(D) + (0.6*\L,0)$)};

\end{tikzpicture}
